A Unified Framework for Automated Code Transformation and Pragma Insertion

High-level synthesis, source-to-source compilers, and various Design Space Exploration techniques for pragma insertion have significantly improved the Quality of Results of generated designs. These tools offer benefits such as reduced development time and enhanced performance. However, achieving high-quality results often requires additional manual code transformations and tiling selections, which are typically performed separately or as pre-processing steps. Although DSE techniques enable code transformation upfront, the vastness of the search space often limits the exploration of all possible code transformations, making it challenging to determine which transformations are necessary. Additionally, ensuring correctness remains challenging, especially for complex transformations and optimizations. To tackle this obstacle, we first propose a comprehensive framework leveraging HLS compilers. Our system streamlines code transformation, pragma insertion, and tiles size selection for on-chip data caching through a unified optimization problem, aiming to enhance parallelization, particularly beneficial for computation-bound kernels. Them employing a novel Non-Linear Programming (NLP) approach, we simultaneously ascertain transformations, pragmas, and tile sizes, focusing on regular loop-based kernels. Our evaluation demonstrates that our framework adeptly identifies the appropriate transformations, including scenarios where no transformation is necessary, and inserts pragmas to achieve a favorable Quality of Results.

==> sources/cnn.tex <==
% % \vspace{-0.10cm}
\begin{figure}[H]
% \vspace{-0.5cm}
\begin{lstlisting}[label={lst:cnn},caption={Code of CNN found by \framework}]
for (i0 = 0; i0 < 16; i0++) { // L0
 load(weight,vweight,i0); // size 16*256*5*5 
 load(output,voutput,i0); // size 16*224*224 
 for (j0 = 0; j0 < 128; j0++) { // L1
  load(input, vinput, j0); // size 2*228*228 
   for (q0 = 0; q0 < 5; q0++) // L2
    for (w0 = 0; w0 < 28; w0++) // L3
     for (h1 = 0; h1 < 224; h1++) // L4
#pragma HLS pipeline
      for (i2 = 0; i2 < 16; i2++)  // L5, unrolled
      for (j2 = 0; j2 < 2; j2++)   // L6, unrolled
      for (w2 = 0; w2 < 8; w2++)   // L7, unrolled
      for (p2 = 0; p2 < 5; p2++){  // L8, unrolled
         h = ...
         output[i2][h][w] +=weight[i2][j][p][q] 
                        * input[j2][h+p][w+q];}}
 store_output(voutput, output, i0);}
\end{lstlisting}
% \vspace{-0.6cm}
\end{figure}
% % \vspace{-0.7cm}

% float output_S0[16][224][224];
%     float input_S0[1][228][228];
%     float weight_S0[16][256][5][5];



==> sources/code_transformation_old.tex <==
\label{sec:code_transformation}


We proceed to develop a methodology that integrates code transformation, tile size selection and pragma insertion into a unified optimization framework. This involves implementing maximal distribution for code transformation, followed by the design and implementation of a template capable of executing code transformation tile size selection and pragma insertion simultaneously. We illustrate our code transformation process step by step using the simple example provided in Listing \ref{lst:example1}.

% \vspace{-0.1cm}

\begin{lstlisting}[label={lst:example1},caption={Code Original of our example}]
for (int i = 0; i < TC_I; i++)
    for (int j = 0; j < TC_J; j++)
        t[i] += A[i][j] * x[j];
\end{lstlisting}
% \vspace{-0.5cm}

\myparagraph{Maximum Distribution}
To kickstart the process, we begin by thoroughly distributing the program, with the goal of maximizing the distance between each statement. This distribution strategy creates ample opportunities for parallelization by maximizing the separation between dependencies.
% 
Typically, this results in one statement per loop body with perfectly nested loops i.e. when loops are entirely contained within another loop without any intervening code between them.
% 
To achieve this, we employ ISCC \cite{iscc} a command line tool bundled with Barvinok \cite{barvinok-web}.
% , showcases a wide range of functionalities, many of which align with those offered by the ISL library \cite{isl}.
It allows us to explore various schedule distributions and validate the legality of transformations by ensuring dependency constraints are preserved. Our example in Listing \ref{lst:example1} is already distributed.

\myparagraph{Strip-mining}
Following maximal distribution, we perform strip-mining on each loop twice. This process replaces the original loop, with a trip count $tc$, with three new loops, each having trip counts $tc_0, tc_1$ and $tc_2$ with $tc_0 \times tc_1 \times tc_2 = tc$.
% 
Since strip mining is inherently legal, there's no necessity to validate the legality of this transformation. 
Subsequently, we can arrange the loops in different permutations if it is legal.

Following the explanation provided in the next paragraph, strip mining allows us to create opportunities for fine-grained unrolling, pipelining, sequential execution,  coarse-grained unrolling and tiling if loop permutation is legal. This expands the range of possibilities, allowing each loop to integrate diverse hardware directives and be reorganized across different levels of the code.

After applying three levels of strip-mining, we transform the original code from Listing \ref{lst:example1} to that depicted in Listing \ref{lst:example2}.

\begin{lstlisting}[label={lst:example2},caption={Code of the example after three level strip-mining}]
for (int i0 = 0; i0 < TC_I_0; i0++)
  for (int i1 = 0; i1 < TC_I_1; i1++)
    for (int i2 = 0; i2 < TC_I_2; i2++)
      for (int j0 = 0; j0 < TC_J_0; j0++)
        for (int j1 = 0; j1 < TC_J_1; j1++)
          for (int j2 = 0; j2 < TC_J_2; j2++) {
            i = i0 * TC_I_1 * TC_I_2 + i1 * TC_I_2 + i2;
            j = j0 * TC_J_1 * TC_J_2 + j1 * TC_J_2 + j2;
            t[i] += A[i][j] * x[j];}
\end{lstlisting}
% \vspace{-0.4cm}

\myparagraph{Loop Permutation}
Following this, we explore potential permutations of the strip-mined loops. If these permutations meet legality criteria, we establish three levels of loops.

The innermost level facilitates fine-grained unrolling (complete unrolling) which increases parallelism by duplicating statements and utilizes tree reduction if a reduction loop is unrolled. 
The middle level facilitates pipelining, enhancing throughput by overlapping loop iterations. 
Finally, the outermost level coordinates coarse-grained unrolling, tiling, and/or sequential execution, optimizing to increase the parallelism, and controlling the size of the on-chip buffer through tiling.
If the loop body consists of only one statement and loop permutation is feasible, we disable coarse-grained unrolling. This will achieve equivalent results because our template permits unrolling the same loop innermost for fine-grained unrolling.
% 
Furthermore, coarse-grained unrolling entails duplicating each array, including read-only arrays, to ensure full overlapping of the modules, even when there are no dependencies between the concurrently executed modules.

% However, if a loop cannot be permuted due to dependencies, typically occurring when maximal distribution does not yield one statement per loop body, the three levels of strip-mined splitting remain unaltered, but the three loops are  consecutive.

In scenarios where permutations enable us to achieve perfectly nested loops capable of being pipelined,
only one loop can usually be pipelined. Trying to pipeline all loops simultaneously, akin to pragma loop\_pipelined, significantly complicates the design and extends synthesis times unreasonably. Thus, if a loop in the middle level is pipelined, it implies that the trip counts of the other loops (in the middle level) are reduced to one, ensuring manageable design complexity and synthesis times.

As explained earlier, loop order selection is not necessary at the pipeline level. However, for the coarse-grained and fine-grained levels, loop order becomes crucial. In the fine-grained level, arranging loops is straightforward; placing the reduction loop innermost enables efficient tree reduction. Conversely, at the coarse-grained or tiled level, prioritizing memory transfer latency is key. Therefore, we opt for a loop order that maintains the output stationary, minimizing costs associated with loading on-chip and storing off-chip during tile iterations, especially when the output is not fully transferred to the chip.

In the context of our example, these transformations yield the code presented in Listing \ref{lst:example3}, with each level corresponding to specific transformations.
% \vspace{-0.1cm}
\begin{lstlisting}[label={lst:example3},caption={Final template of our example}]
// possibilities to cache on-chip t, A and x
/********* Level 0 *********/
for (int i0 = 0; i0 < TC_I_0; i0++)
// possibilities to cache on-chip t and A
  for (int j0 = 0; j0 < TC_J_0; j0++)
// possibilities to cache on-chip A and x
/********* Level 1 *********/
    for (int i1 = 0; i1 < TC_I_1; i1++)
#pragma HLS pipeline // if T_J_1 = 1
      for (int j1 = 0; j1 < TC_J_1; j1++)
#pragma HLS pipeline // if T_I_1 = 1
/********* Level 2 *********/
        for (int i2 = 0; i2 < TC_I_2; i2++)
#pragma HLS unroll // fine-grained unrolled
          for (int j2 = 0; j2 < TC_J_2; j2++) {
#pragma HLS unroll // fine-grained unrolled
            i = i0 * TC_I_1 * TC_I_2 + i1 * TC_I_2 + i2;
            j = j0 * TC_J_1 * TC_J_2 + j1 * TC_J_2 + j2;
            t[i] += A[i][j] * x[j];}
\end{lstlisting}
% \vspace{-0.5cm}

\myparagraph{Fusion}
We have opted not to incorporate fusion into our model for several reasons. Firstly, our objective is to maximize parallelization for computation-bound kernels. Fusion may reduce or minimize the dependencies distance between statements, limiting potential parallelization opportunities. Additionally, since our focus is on computation-bound kernels, the primary bottleneck lies in computation. Therefore, we are willing to incur a minor cost, even if it involves transferring a tiled array multiple times.

% % \vspace{-0.08cm}

\myparagraph{Space}
Therefore, the challenge involves determining the trip counts of each loop (e.g., $TC\_I\_0$).
Additionally, the design must adhere to resource constraints, including the usage of DSP and on-chip memory. Hence, the trip counts corresponding to fully unrolled loops must be constrained to avoid over-utilization of DSP resources. The on-chip buffers must not exceed the on-chip memory capacity. Consequently, for a large problem size, the outermost level will enable control over the buffer sizes.
% 
% Need to give an intuition of the space TODO
% 
Thus, the space we consider encompasses the original schedule on which we can insert pragmas, but it also includes all the transformations mentioned previously for which the pragmas are inserted.

==> sources/eq.tex <==
% \vspace{-0.4cm}

\begin{eqnarray}
% \left\{
% \label{eq:TC_init}
%  \forall l \in \mathcal{L}, \forall v \in \mathcal{V}, 1 \leq TC_{l, v} \leq TC_l
% \\
\label{eq:TC}
 \forall l \in \mathcal{L}, \prod_{v \in \mathcal{V}} TC_{l, v} = TC_l
\\
\label{eq:loop_uf_less_than_tc}
 \forall l \in \mathcal{L}, loop_l\_UF \leq TC_{l, 0} 
\\
\label{eq:uf_if_perfectly}
\forall s \in \mathcal{S}_1, \forall l \in \mathcal{L}_s, loop_l\_UF = 1 \\
\label{eq:uf_if_seq}
\forall s \in \mathcal{S}_1, \forall l \in \mathcal{L}_s^{red}, loop_l\_UF = 1
\\
\label{eq:uf_divide_tc}
% \begin{cases}
\forall l \in \mathcal{L}, loop_l\_UF \% TC_{l,0} == 0
% \end{cases}
\\
\label{eq:pip}
\forall l \in \mathcal{L}, loop_l\_pip \in \{0,1\}
\\
\label{eq:pip2}
\forall l \in \mathcal{L}, (1-loop_l\_pip) \times TC_{l,1} == 1
\\
\label{eq:one_pip_per_nesteed_loop}
% \begin{cases}
\forall s \in \mathcal{S}, \sum_{l \in \mathcal{L}_s} loop_l\_pip \leq 1
% \end{cases}
\\
\label{eq:II}
\forall s \in \mathcal{S}, II_s = \sum_{l \in \mathcal{L}_s} loop_l\_pip \times II_l 
\\
\label{eq:cache}
\forall l \in \mathcal{L}, \forall a \in \mathcal{A}, cache_l\_arr_a \in \{0,1\}
\\
% \label{eq:foot}
% \begin{cases}
%     & \sum_{a \in \mathcal{A}} \sum_{l \in \mathcal{L}} cache_l\_arr_a \\ & \times ft\_array_a\_loop_l \leq Mem
% \end{cases}
% \\
\label{eq:foot}
 \sum_{a \in \mathcal{A}} \sum_{l \in \mathcal{L}} cache_l\_arr_a   \times ft\_array_a\_loop_l \leq Mem
\\
\label{eq:max_part1}
\forall a \in \mathcal{A}, \prod_{d \in \mathbb{N}} 
AP_{a,d} \leq max_{part} \\
\label{eq:max_part2}
\forall a \in \mathcal{A}, \forall d \in \mathbb{N}, \forall l \in C_{a_d}, 
AP_{a,d} \% TC_{l,2} == 0 \\
\label{eq:max_part3}
\forall a \in \mathcal{A}, \forall d \in \mathbb{N}, \forall l \in C_{a_d}, 
AP_{a,d} \geq TC_{l,2} \\
\label{eq:dsp_optimistic}
 DSPs\_used_{opt} = 
     \sum_{op \in \{+,-,*,/ \}} \max_{s \in \mathcal{S}}(DSP_{s_{op}} / II_s) 
\\
\label{eq:dsp_pessimist}
 DSPs\_used_{pes} = 
     \sum_{op \in \{+,-,*,/ \}} \sum_{s \in \mathcal{S}}(DSP_{s_{op}} / II_s) 
\\
\label{eq:dsp1}
reuse_{opt} \times DSPs\_used_{opt}  \leq DSP_{available} \\
\label{eq:dsp2}
 (1-reuse_{opt}) \times DSPs\_used_{pes} \leq DSP_{available} \\
\nonumber % to remove the +1 label without equation
\end{eqnarray}

% \vspace{-0.5cm}

==> sources/gemm_autodse.tex <==


% % \vspace{-0.2cm}
\begin{figure}[H]
% \vspace{-0.4cm}
\begin{lstlisting}[label={lst:gemm_motiv_autodse},caption={Code of gemm found by AutoDSE},escapeinside={(*@}{@*)}]
(*@\tiny \#pragma ACCEL parallel factor=1@*)
(*@\tiny \#pragma ACCEL pipeline off@*)
#pragma ACCEL TILE FACTOR=5
for (i = 0; i < 200; i++) { // L0
(*@\tiny \#pragma ACCEL tile factor=1@*)
(*@\tiny \#pragma ACCEL pipeline off@*)
#pragma ACCEL parallel FACTOR=4
  for (j = 0; j < 220; j++) // L1
    C[i][j] *= beta; // S0
(*@\tiny \#pragma ACCEL tile factor=1@*)
(*@\tiny \#pragma ACCEL parallel factor=1@*)
#pragma ACCEL pipeline flatten
  for (k = 0; k < 240; k++)  // L2
(*@\tiny \#pragma ACCEL pipeline off@*)
(*@\tiny \#pragma ACCEL tile factor=1@*)
#pragma ACCEL parallel factor=220
    for (j = 0; j < 220; j++) // L3
      C[i][j] += alpha * A[i][k] * B[k][j];} // S1
\end{lstlisting}
% \vspace{-0.6cm}
\end{figure}
% % \vspace{-0.6cm}


==> sources/gemm_code.tex <==
% % \vspace{-0.1cm}
\begin{figure}
\begin{lstlisting}[label={lst:gemm_motiv},caption={Code of gemm found by \framework}]
// possibilities to cache on-chip A, B and C
/********* Level 0 *********/
for (int i0 = 0; i0 < 1; i0++) // L0
// possibilities to cache on-chip C
 for (int j0 = 0; j0 < 1; j0++) // L1
// possibilities to cache on-chip C
/********* Level 1 *********/
  for (int j1 = 0; j1 < 1; j1++) // L2
   for (int i1 = 0; i1 < 50; i1++) // L3
#pragma HLS pipeline
/********* Level 2 *********/
    for (int i2 = 0; i2 < 4; i2++) // L4
#pragma HLS unroll
     for (int j2 = 0; j2 < 220; j2++) // L5
#pragma HLS unroll
      C[i1*4+i2][j2] *=beta; // S0
/********* Level 0 *********/
for (int i0 = 0; i0 < 1; i0++) // L6
// possibilities to cache on-chip A and C
 for (int j0 = 0; j0 < 1; j0++) // L7
// possibilities to cache on-chip B and C
  for (int k0 = 0; k0 < 80; k0++) // L8
// possibilities to cache on-chip A and B
/********* Level 1 *********/
   for (int j1 = 0; j1 < 1; j1++) // L9
    for (int k1 = 0; k1 < 1; k1++) // L10
     for (int i1 = 0; i1 < 200; i1++) // L11
#pragma HLS pipeline
/********* Level 2 *********/
      for (int i2 = 0; i2 < 1; i2++) // L12
#pragma HLS unroll
       for (int j2 = 0; j2 < 220; j2++) // L13
#pragma HLS unroll
        for (int k2 = 0; k2 < 3; k2++) // L14
#pragma HLS unroll
         i = i0 * 200 + i1 * 1 + i2;
         j = j0 * 220 + j2; k = k0 * 3 + k2;
         C[i][j] +=alpha*A[i][k] * B[k][j]; // S1
\end{lstlisting}
\end{figure}
% % \vspace{-0.6cm}




==> sources/gemm_distributed.tex <==


\begin{lstlisting}[label={lst:gemm_distributed},caption={Code of gemm Distributed}]
for (i = 0; i < 200; i++) 
  for (j = 0; j < 220; j++)
    C[i][j] *= beta;
for (i = 0; i < 200; i++) 
  for (k = 0; k < 240; k++) 
    for (j = 0; j < 220; j++) 
      C[i][j] += alpha * A[i][k] * B[k][j];}
\end{lstlisting}
% \vspace{-0.5cm}

==> sources/gemm_original.tex <==

% % \vspace{-0.1cm}
\begin{figure}
\begin{lstlisting}[label={lst:gemm_motiv_ori},caption={Code original of gemm}]
for (i = 0; i < 200; i++) { // L0
  for (j = 0; j < 220; j++) // L1
    C[i][j] *= beta; // S0
  for (k = 0; k < 240; k++) // L2
    for (j = 0; j < 220; j++)  // L3
      C[i][j] += alpha*A[i][k] * B[k][j];} // S1 
\end{lstlisting}
\end{figure}
% % \vspace{-0.6cm}

% \begin{figure}[h]
%   \centering
%   \begin{minipage}{0.48\textwidth}
%     \begin{lstlisting}[label={lst:gemm_motiv_ori},caption={Original gemm code}]
% for(i=0;i<200;i++){//L0
%  for(j=0;j<220;j++)//L1
%   C[i][j]*=beta;//S0
%  for(k=0;k<240;k++)//L2
%   for(j=0;j<220;j++)//L3
%    C[i][j]+=alpha*A[i][k]*B[k][j];}//S1 
%     \end{lstlisting}
%   \end{minipage}
%   % \hfill
%   \begin{minipage}{0.48\textwidth}
%     \begin{lstlisting}[label={lst:gemm_motiv_opt},caption={Optimized gemm code}]
% for(i=0;i<200;i++){//L0
%  for(k=0;k<240;k++)//L1
%   for(j=0;j<220;j++)//L2
%    C[i][j]+=alpha*A[i][k]*B[k][j];}//S0
% for(i=0;i<200;i++)//L3
%  for(j=0;j<220;j++)//L4
%   C[i][j]*=beta;//S1 
%     \end{lstlisting}
%   \end{minipage}
%   \caption{Comparison of original and optimized gemm code}
% \end{figure}

==> sources/gemm_strip.tex <==



\begin{figure}
\begin{lstlisting}[label={lst:gemm_distributed},caption={Code of the first loop body of gemm with three level strip mining}]
for (i0 = 0; i0 < TC_I0_0; i0++) 
 for (i1 = 0; i1 < TC_I0_1; i1++) 
  for (i2 = 0; i2 < TC_I0_2; i2++) 
   for (j0 = 0; j0 < TC_J0_0; j0++)
    for (j1 = 0; j1 < TC_J0_1; j1++)
     for (j2 = 0; j2 < TC_J0_2; j2++)
      i = i0*TC_I0_1*TC_I0_2 + i1*TC_I0_2 + i2; 
      ...
      C[i][j] *= beta;
\end{lstlisting}
\end{figure}

% for (i0 = 0; i0 < TC_I1_0; i0++)
%  for (i1 = 0; i1 < TC_I1_1; i1++)
%   for (i2 = 0; i1 < TC_I1_2; i2++)
%    for (k0 = 0; k0 < TC_K1_2; k0++)
%     for (k1 = 0; k1 < TC_K1_2; k1++)
%      for (k2 = 0; k2 < TC_K1_2; k2++)
%       for (j0 = 0; j0 < TC_J1_0; j0++)
%        for (j1 = 0; j1 < TC_J1_1; j1++)
%         for (j2 = 0; j2 < TC_J1_2; j2++)
%          i = i0 * TC_I0_1 * TC_I0_2 + i1 * TC_I0_2 + i2;
%          ...
%          C[i][j] += alpha * A[i][k] * B[k][j];}

==> sources/gemm_template.tex <==
% % \vspace{-0.1cm}
\begin{figure}
\begin{lstlisting}[label={lst:gemm_template},caption={Template of gemm}]
// INPUT: int perm[2] Array to store permutation order (0 for i0, 1 for j0)
// INPUT: int perm_S1[3] Array to store permutation order (i0, j0, k0)
int lb_S1[3] = {I0_S1, J0_S1, K0_S1}; // Store loop bounds for S1
int lb_S0[2] = {I0_S0, J0_S0}; // Store loop bounds
// possibilities to cache on-chip A, B and C
/********* Level 0 of S0 *********/
for (int L0_S0 = 0; L0_S0 < lb_S0[perm_S0[0]]; L0_S0++) { 
// possibilities to cache on-chip A, B and C
 for (int L1_S0 = 0; L1_S0 < lb_S0[perm_S0[1]]; L1_S0++) { 
 // possibilities to cache on-chip A, B and C
/********* Level 1 of S0 *********/
  for (int j1 = 0; j1 < J1_S0; j1++) // L2
   for (int i1 = 0; i1 < I1_S0; i1++) // L3
#pragma HLS pipeline
/********* Level 2 of S0 *********/
    for (int i2 = 0; i2 < I2_S0; i2++) // L4
#pragma HLS unroll
     for (int j2 = 0; j2 < J2_S0; j2++) // L5
#pragma HLS unroll
      C[i1*4+i2][j2] *=beta; // S0
/********* Level 0 of S1 *********/
for (int L0_S1 = 0; L0_S1 < lb_S1[perm_S1[0]]; L0_S1++) 
// possibilities to cache on-chip A, B and C
 for (int L1_S1 = 0; L1_S1 < lb_S1[perm_S1[1]]; L1_S1++) 
 // possibilities to cache on-chip A, B and C
  for (int L2_S1 = 0; L2_S1 < lb_S1[perm_S1[2]]; L2_S1++) 
  // possibilities to cache on-chip A, B and C
/********* Level 1 of S1 *********/
   for (int j1 = 0; j1 < J1_S1; j1++) // L9
    for (int k1 = 0; k1 < K1_S1; k1++) // L10
     for (int i1 = 0; i1 < I1_S1; i1++) // L11
#pragma HLS pipeline
/********* Level 2 of S1 *********/
      for (int i2 = 0; i2 < I2_S1; i2++) // L12
#pragma HLS unroll
       for (int j2 = 0; j2 < J2_S1; j2++) // L13
#pragma HLS unroll
        for (int k2 = 0; k2 < K2_S1; k2++) // L14
#pragma HLS unroll
         i = i0 * I1_S1 * I2_S1 + i1 * I2_S1 + i2;
         j = j0 * J1_S1 * J2_S1 + j1 * J2_S1 + j2; 
         k = k0 * K1_S1 * K2_S1 + k1 * K2_S1 + k2; 
         C[i][j] +=alpha*A[i][k] * B[k][j]; // S1
\end{lstlisting}
\end{figure}

==> sources/longtable.tex <==


% \begin{longtable}[!htb]
\begin{longtable}[H]

% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{0.18\linewidth}p{0.82\linewidth}@{}}
\toprule
Set & Description \\
\midrule
$\mathcal{L},\mathcal{A},\mathcal{S}$ & the set of loops, arrays and statements \\
$\mathcal{S}_{1}$ & the set of statements alone in a loop body \\
$\mathcal{O}_s$ & the list of operations of the statements $s$ \\
% $\mathcal{O}_{s_{par}}$ & the operation which can be done in parallel, i.e., does not have any loop-carried dependence \\ 
$\mathcal{L}_s$ &  the set of nested loops which iterate the statement $s$ \\
$\mathcal{L}_s^{red}$ &  the set of reduction loops which iterate the statement $s$ \\
$\mathcal{C}_{a_d}$ & the set of loops which iterates the array $a$ at the dimension $d$ \\ 
$\mathcal{V}$ & Level of the strip mining, 0 for coarse-grained/sequential, 1 for pipeline and 2 for fine-grained unrolled \\
$AP_{a,d}$ & Array Partition for the array $a$ in dimension $d$ \\
% $d_l$ & the maximum dependency distance of the loop $l$ \\
\midrule
Variable & Description \\
\midrule

$tc_{l, level}$ & TC of the loop $l$ for the level of strip-mining \\
$loop_l\_UF$ & Coarse-grained unroll factor of the loop $l$ at level 0 of the strip-mining\\
$loop_l\_pip$  & Boolean to know if the loop $l$ is pipelined at level 1 of the strip-mining\\
$cache_l\_arr_a$ & Boolean to know if the array $a$ is transferred on-chip after the loop $l$ at level 0 of the strip-mining \\
\midrule
Constant & Description \\
\midrule
$TC_l$ & Trip Count of the loop $l$ before strip-mining \\
$II_l$ & II of the loop $l$ \\
$IL_{par}, IL_{red}$ & Iteration Latency of the operations without ($par$) and with ($red$) dependencies of the statement $s$\\
% $IL_{red}$ & Iteration Latency of the operations with dependencies of the statement $s$\\
$DSP_{s_{op}}$ & Number of DSP used for the statement $s$ for the operation $op$\\
$DSP_{available}$ & Number of DSP available for the FPGA used \\
$max_{part}$ & Maximum array partitioning defined by the user \\
$ft\_arr_a\_loop_l$ & Footprint of the array $a$ if transferred to on-chip before the loop $l$ \\
$reuse_{opt}$ & Boolean for optimistic reuse \\
\bottomrule
\end{tabular}%
% }
\caption{Overview of the sets, variables, and constants employed in formulating the NLP}
\label{tab:var}
\end{longtable}

% \vspace{-0.4cm}

==> sources/motivation_old.tex <==
\label{sec:motivation}



\subsection{Space to explore}

The exploration space for optimizing an HLS design encompasses pragma insertion, code transformation, and data caching, all while adhering to resource constraints. While various objective functions can be considered, our focus in this work is on minimizing latency by maximizing parallelism. 
This objective function is especially potent for computation-bound kernels, addressing the bottleneck caused by insufficient parallelization.
% 
These different elements of the space (pragma insertion, code transformation, and data caching) are inherently interconnected. Inserting unrolled pragmas influences array partitioning and thus the utilization of BRAM. The schedule and pragmas influence the possibility of caching data on-chip, and the choice of schedule impacts how we want to unroll based on loop properties (e.g., reduction loop), and so on. Thus, the choice of one element affects the others, necessitating backtracking if the spaces are separated. This complexity complicates the exploration of the space and also requires constant verification of the legality of transformations.

\subsection{Limitation of the current DSE}

Several frameworks \cite{heterocl, scalehls, zhaopolsca} enable code transformations and pragma insertion, but their spaces are limited for both. 
% 
Transformations are restricted to loop property-based permutations or the use of Pluto \cite{pluto}, which tiles the program but may restrict parallelization for FPGAs and does not consider FPGA-specific optimizations such as pipelining or array partitioning.

On the other hand, numerous Design Space Explorations (DSEs) \cite{autodse, harp, sohrabizadeh2022gnn, nlp_dse} explore pragma insertion for a fixed loop order. Although the user may initially set the schedule, it can be difficult, even for experts, to predict which transformations are necessary prior to pragma insertion. 
Furthermore, the multitude of code transformations renders the exploration of each pragma impractical in terms of scalability.

We will now examine examples that highlight the limitations of current methods.
For this, we use two different downstream HLS DSE methods, AutoDSE \cite{autodse} and NLP-DSE \cite{nlp_dse}. 
% 
AutoDSE trents the compiler Merlin \cite{merlin} as a black box, adjusting pragmas based on identified bottlenecks from previous iterations. In contrast, NLP-DSE employs Nonlinear Programming DSE, utilizing a lower bound-based objective function to achieve high QoR within a short timeframe.

% to explore various theoretical subspaces efficiently, aiming to achieve a high QoR within a short timeframe.
% 
Table \ref{tab:motivation} presents a comparison of two pragma insertion DSE methods against \framework for the kernels atax, bicg, CNN, and gemm synthesized with tree reduction, as well as gemm$^{*}$ synthesized without tree reduction.

% % \vspace{-0.30cm}
% \vspace{-0.2cm}
\begin{table}[H]
    \centering
\begin{tabular}{@{}l rr  r  @{}}
\toprule
    % & \multicolumn{3}{c}{GF/s} \\
    \cmidrule{2-4}
      Kernel   & GF/s AutoDSE &  GF/s NLP-DSE &  GF/s \framework \\
      \midrule
        atax &  1.98 &	1.96 &	1.96    \\
        bicg & 0.99 & 0.99 & 1.96 \\
        % \midrule
        
        % \midrule
        gemm &  110.81 &	131.32 &	198.26    \\
        gemm$^{*}$  & 22.77&		22.01 &		210.63          \\
        CNN &  42.55 &	38.19	& 340.20      \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of the Throughput (GF/s) achieved with AutoDSE, NLP-DSE and \framework }
    \label{tab:motivation}
\end{table}
% \vspace{-0.8cm}


\myparagraph{Computation bound kernel}
For computation bound kernel they need to increase the parallelism to have a good QoR.
% For gemm, as shown in Listing \ref{lst:gemm_motiv_ori}, the benefits of code transformation are apparent. 
Using the original schedule and tree reduction, both AutoDSE and NLP-DSE were able to partially unroll and pipeline the reduction loop of gemm, resulting in a satisfactory QoR. However, when tree reduction is absent (gemm$^{*}$), a performance decrease happens because of the inability to partially unroll the reduction loop, Listing \ref{lst:gemm_motiv_ori} shows the design discovered by AutoDSE. In such cases, a transformation becomes essential.

\input{sources/gemm_original}

\myparagraph{Computation bound kernel with need of tiling}
Regarding CNN, the potential for code transformation is vast, especially considering the necessity for tiling. The permutations of each loop split once yield an immense number of possibilities, reaching $2.23 \times 10^{13}$ possible schedule. Despite achieving satisfactory QoR, both methods fail to fully exploit the available level of parallelism, indicating potential for further optimization. However, exploring each code transformation is practically infeasible due to the sheer number of possibilities. 
While the Merlin compiler, a source-to-source tool, can perform code transformation such as strip mining to enhance the potential for on-chip data caching, its capabilities in this regard are limited.

\myparagraph{Memory bound kernel}
Disregarding initialization, atax and bicg share kernel similarities as they both consist of two statements.
Each statement iterates through a reduction loop and a non-reduction loop. Notably, in atax, the two statements are interdependent.
% 
Both kernels are memory-bound bound because of the array $A$. The statements of the kernel atax are already distributed. While loop reordering based on properties could be used, atax's memory-bound nature and the distinct dimensions of the reduction loops in the two statements render loop permutation impractical resulting from array partitioning constraints. Consequently, the most efficient strategy for minimizing latency is to retain one reduction loop innermost and another outermost, a configuration which is already inherent in the original code.
% 
In the original schedule of bicg the statements are consecutive in order to minimize the RaR dependencies of array $A$, which prevent an efficient parallelization. 
% By applying distribution and the good loop order to parallelize the array $A$ on the same dimension we found a similar case to atax.




\subsection{Overview of \framework}


To address these limitations, we propose \framework, which focuses on linear code to offer a space capable of exploring only legal code transformations, pragma insertions, and tile size selections as a single optimization problem. Leveraging a Nonlinear Programming (NLP) approach, \framework can efficiently explore this space, benefiting from accurate modeling enabled by compile-time analysis feasible for linear code. The space comprises three levels of tiling, each corresponding to a specific optimization: fine-grained unrolling, pipelining, and coarse-grained unrolling, with loops executed sequentially and data transferred between off-chip and on-chip.

Let's analyze the previous examples.

\myparagraph{Code transformation for computation bound kernel}
For gemm, \framework demonstrates the capability to enhance throughput. The NLP selects a schedule that partially unrolls the three loops and pipelines the reduction loop, resulting in improved QoR. 
Pipelining the reduction loop does not enable pipelining with an initiation interval of 1 (II=1), but it does reduce resource consumption in the unrolled portion.
% 
Notably, when tree reduction is not employed (gemm$^*$), \framework excels by splitting and permuting the loops to enhance parallelism without relying on the reduction loop. In this scenario, the NLP finds the configuration presented on Listing \ref{lst:gemm_motiv}. The reduction loop is partially unrolled, enabling the two multiplications to be performed in parallel.

\input{sources/gemm_code}

\myparagraph{Ability to keep the schedule when it is needed}
\framework adeptly preserves the existing loop order for atax while precisely inserting the necessary pragmas. As discussed in Section \ref{sec:evaluation}, we observe a slight decrease in performance compared to AutoDSE, mainly because the best design found by AutoDSE is excluded from our space due to array partitioning exceeding 1024 (the limit set by the HLS compiler we used). Consequently, our framework retains the original schedule while only inserting pragmas.

\myparagraph{Code transformation for memory bound kernel}
By maximally distributing statements and implementing an efficient loop order that facilitates unrolling the loop iterating over the same dimension as the array $A$, bicg demonstrates a comparable scenario to atax.
This adjustment enables a doubling of throughput, enhancing overall performance.

\myparagraph{Code transformation for computation bound kernel with need of tiling}
Regarding CNN, the NLP swiftly identifies a solution in 4.5 minutes. This solution optimizes tile configuration, caching a data tile of the array on-chip, partially unrolling one reduction loop and two non-reduction loops, and pipelining a non-reduction loop, resulting in a design with 340 GF/s.





% In Section \ref{sec:code_transformation}, we elaborate on the transformations facilitated by our framework. Section \ref{sec:nlp} delves into the model utilized to navigate the space effectively. Lastly, Section \ref{sec:code_generation} outlines our code generation process, including the post-optimization techniques employed to address communication overlapping concerns.

==> sources/symm_code_if_needed.tex <==


\begin{lstlisting}[label={lst:symm_motiv},caption={Symm code: $C=\alpha \times A \times B + \beta \times C$}]
L0: for (i = 0; i < 200; i++) {
  L1: for (j = 0; j < 240; j++) {
    S0: temp2[i][j] = 0.0;
    L2: for (k = 0; k < i; k++) {
      S1: C[k][j] += alpha * B[i][j] * A[i][k];
      S2: temp2[i][j] += B[k][j] * A[i][k];
    }
    S3: C[i][j] = beta * C[i][j] 
                  + alpha * B[i][j] * A[i][i] 
                  + alpha * temp2[i][j];
  }
}
\end{lstlisting}

\begin{lstlisting}[label={lst:symm_motiv2},caption={Symm code after maximal distribution}]
L0: for (i = 0; i < 200; i++)
  L1: for (j = 0; j < 240; j++)
    S0: temp2[i][j] = 0;
L2: for (i = 0; i < 200; i++) 
  L3: for (j = 0; j < 240; j++) 
    L4: for (k = 0; k < 199; k++) 
      C0: if (k < i)
        S1: temp2[i][j] += B[k][j] * A[i][k];
L5: for (i = 0; i < 200; i++) 
  L6: for (j = 0; j < 240; j++) 
    S2: C[i][j] = beta * C[i][j] 
                  + alpha * B[i][j] * A[i][i] 
                  + alpha * temp2[i][j];
L7: for (i = 0; i < 200; i++) 
  L8: for (j = 0; j < 240; j++) 
    L9: for (k = 0; k < 199; k++) 
      C1: if (k<i)
        S3: C[k][j] += alpha * B[i][j] * A[i][k];
\end{lstlisting}

\begin{lstlisting}[label={lst:comp_motiv},caption={Computation for statement iterated by loop with non-constant trip count}]
float computation(float C, float alpha, float B, float A, int i, int k){
    if (k<i)
        return C+alpha*B*A;
    else:
        return C;
}
\end{lstlisting}

==> sources/table.tex <==
% \vspace{-0.22cm}
\begin{table}[H]
\begin{adjustwidth}{-1in}{-1in}
    
\centering
\begin{tabular}{@{}l @{\hspace{-1mm}}rr  r rr @{}}
\toprule
& &  \multicolumn{1}{l}{GF/s} & & \multicolumn{2}{l}{Perf. Improvement} \\
\cmidrule{3-3}
\cmidrule{5-6}

\textbf{Kernel} &  \textbf{Tree Red.} & 
% \textbf{AutoDSE} & \textbf{NLP-DSE} & 
\textbf{Sisyphus} & & \textbf{AutoDSE} & \textbf{NLP-DSE}  \\

\midrule
2mm & True & 164.34 &  & 403.55x & 1.33x\\
atax & True & 1.96 &  & 0.99x & 1.00x\\
bert\_100\_3072 & True & 220.29 &  & 1.10x & 1.10x\\
bert\_100\_64 & True & 88.30 &  & 1.08x & 1.03x\\
bert\_100\_768 & True & 218.08 &  & 1.04x & 1.10x\\
bert\_3072\_100 & True & 42.93 &  & 2.98x & 3.31x\\
bicg & True & 1.96 &  & 1.97x & 1.97x\\
cnn & True & 340.20 &  & 8.00x & 8.91x\\
doitgen & True & 53.22 &  & 1.33x & 2.66x\\
gemm & True & 198.26 &  & 1.79x & 1.51x\\
gemver & True & 17.85 &  & 4.64x & 1.77x\\
mvt & True & 13.71 &  & 1.76x & 1.76x\\
symm & True & 236.82 &  & 8.15x & 7.20x\\
syr2k & True & 428.12 &  & 9.28x & 3.12x\\
syrk & True & 306.07 &  & 12.44x & 4.40x\\
\midrule
2mm & False & 162.24 &  & 775.26x & 1.36x\\
atax & False & 1.86 &  & 0.98x & 1.00x\\
bert\_100\_3072 & False & 219.97 &  & 1.11 & 1.11x\\
bert\_100\_64 & False & 76.76 &  & 1.09x & 1.09x\\
bert\_100\_768 & False & 216.95 &  & 1.13x & 1.13x\\
bert\_3072\_100 & False & 44.67 &  & 536.42x & 626.60x\\
bicg & False & 1.86 &  & 1.92x & 1.93x\\
cnn & False & 307.78 &  & 7.30x & 9.68x\\
doitgen & False & 54.05 &  & 5.46x & 2.71x\\
gemm & False & 210.63 &  & 9.25x & 9.57x\\
gemver & False & 12.45 &  & 30.91x & 7.24x\\
mvt & False & 10.00 &  & 1.45x & 1.45x\\
symm & False & 236.56 &  & 8.14x & 7.19x\\
syr2k & False & 428.39 &  & 17.57x & 3.13x\\
syrk & False & 308.71 &  & 12.55x & 4.43x\\
\midrule
heat-3d & - & 131.33 &  & 35.09x & 0.99x\\
jacobi-2d & - & 128.83 &  & 13.06x & 6.60x\\
\midrule
Average &  & 152.66 &  & 59.96x & 22.79x\\
Geo Mean &  & 68.88 &  & 5.96x & 2.87x\\



\bottomrule

\end{tabular}
\caption{Comparison of the Throughput (GF/s) achieved with \framework, AutoDSE and NLP-DSE }

\label{tab:eval}
\end{adjustwidth}
\end{table}

% \vspace{-0.8cm}





==> sources/table2.tex <==

\begin{table*}[!htb]
\begin{adjustwidth}{-1in}{-1in}
    
\centering
% \begin{tabular}{@{}lll rrr  rr llll lll @{}}
% \begin{tabularx}{0.5\linewidth}{@{}lll rrr  rr llll lll @{}}
\begin{tabular}{ llp{1cm} r  rr p{1cm}p{1cm}p{1cm}p{1cm}  p{1cm} }
\toprule
% & &  \multicolumn{1}{l}{GF/s} & & \multicolumn{2}{l}{Perf. Improvement} \\
% \cmidrule{3-3}
% \cmidrule{5-6}

\textbf{Kernel} &  \textbf{T Red.} & 
\textbf{Pb. Size} & 
% gf/s
% \textbf{A} & 
% \textbf{N} & 
\textbf{S} & 
%perf improvement
 \textbf{A} & 
 \textbf{N}  &
 % perm
  \textbf{S0} & 
 \textbf{S1}  &
  \textbf{S2} & 
 \textbf{S3}  \\
% resource
% \textbf{AutoDSE} & 
% \textbf{NLP-DSE} & 
\textbf{Sisyphus} \\

\midrule
2mm & True & NI 180, NJ 190, NK 210,NL 220 & 164.34 & 403.55 & 1.33 & i1: 36 i2: 5 j2: 190  & i0: 36 k1: 42 i2: 5 j2: 190 k2: 5  & i0: 6 j1: 11 i2: 30 j2: 20  & i0: 36 j1: 220 i2: 5 k2: 190  & 89,0,89,57,0\\
atax & True & M 390, N 410 & 1.96 & 0.99 & 1.00 & i1: 2 i2: 205 & i1: 2 i2: 195 & i: 390 j: 410 & i1: 195 j2: 410 i2: 2  & 59,19,28,25,0\\
bert\_100\_3072 & True & I 100 J 3072 K 100 & 220.29 & 1.10 & 1.10 & j0: 192 i1: 2 i2: 50 j2: 16  & i0: 2 k0: 5 j1: 3072 i2: 50 k2: 20  &  &  & 73,42,49,32,0\\
bert\_100\_64 & True & I 100 J 64 K 100 & 88.30 & 1.08 & 1.03 & i0: 5 i1: 2 i2: 10 j2: 64  & k0: 10 i1: 50 i2: 2 j2: 64 k2: 10  &  &  & 93,1,53,38,0\\
bert\_100\_768 & True & I 100 J 768 K 100 & 218.08 & 1.04 & 1.10 & j0: 48 i1: 2 i2: 50 j2: 16  & i0: 2 k0: 5 j1: 768 i2: 50 k2: 20  &  &  & 73,1,68,38,0\\
bert\_3072\_100 & True & I 3972 J 100 K 3972 & 42.93 & 2.98 & 3.31 & i0: 256 load: C j1: 5 i2: 12 j2: 20  & i0: 64 load: A load: C j0: 5 k1: 3072 i2: 48 j2: 20  &  &  & 11,14,16,8,0\\
bicg & True & M 390, N 410 & 1.96 & 1.97 & 1.97 & i1: 2 i2: 195 & i1: 2 i2: 205 & j1: 195 j2: 2 i2: 410  & j1: 195 i2: 410 j2: 2 & 59,19,28,25,0\\
cnn & True & I 256 J 256 H 224 W 224 P 5 Q 5 & 340.20 & 8.00 & 8.91 & i0: 16 load: weight load: output j0: 256 load: input p0: 5 w0: 14 h1: 224 i2: 16 w2: 16 q2: 5  &  &  &  & 93,8,45,36,0\\
doitgen & True & NQ 40, NR 50, NP 60 & 53.22 & 1.33 & 2.66 & r0: 2 q0: 4 p1: 15 r2: 25 q2: 10 p2: 4  & r0: 2 q0: 4 s0: 15 p1: 60 r2: 25 q2: 10 s2: 4  & q0: 4 p0: 15 r1: 2 r2: 25 q2: 10 p2: 4 &  & 73,0,64,40,0\\
gemm & True & NI 200, NJ 220, NK 240 & 198.26 & 1.79 & 1.51 & i0: 5 j1: 11 i2: 40 j2: 20  & i0: 5 j0: 11 k1: 40 i2: 40 j2: 20 k2: 6  &  &  & 60,3,63,37,0\\
gemver & True & N 400 & 17.85 & 4.64 & 1.77 & i1: 400 j2: 400  & j1: 200 i2: 400 j2: 2  & i1: 2 i2: 200  & j0: 2 i1: 200 i2: 2 j2: 200  & 58,24,44,34,0\\
mvt & True & N 400 & 13.71 & 1.76 & 1.76 & i1: 200 i2: 2 j2: 400  & j1: 200 i2: 400 j2: 2  &  &  & 58,21,27,25,0\\
symm & True & M 200, N 240 & 236.82 & 8.15 & 8.15 &  &  &  &  & 95,10,73,54,0\\
syr2k & True & M 200, N 240 & 428.12 & 9.28 & 3.12 &  &  &  &  & 97,1,86,65,0\\
syrk & True & M 200, N 240 & 306.07 & 12.44 & 4.40 &  &  &  &  & 96,6,48,45,0\\
2mm & False & NI 180, NJ 190, NK 210,NL 220 & 162.24 & 775.26 & 1.36 & i1: 45 i2: 4 j2: 190  & k0: 105 i1: 90 i2: 2 j2: 190 k2: 2  & i1: 90 i2: 2 j2: 220  & k0: 95 i1: 90 i2: 2 j2: 220 k2: 2  & 64,3,72,40,0\\
atax & False & M 390, N 410 & 1.86 & 0.98 & 1.00 & i1: 2 i2: 205  & i1: 2 i2: 195  & i1: 195 i2: 2 j2: 410  & i1: 195 j2: 410 i2: 2 & 29,19,17,16,0\\
bert\_100\_3072 & False & I 100 J 3072 K 100 & 219.97 & 1.11 & 1.11 & j0: 192 i1: 2 i2: 50 j2: 16  & i0: 2 k0: 5 j1: 3072 i2: 50 k2: 20  &  &  & 73,34,46,30,0\\
bert\_100\_64 & False & I 100 J 64 K 100 & 76.76 & 1.09 & 1.09 & i1: 10 i2: 10 j2: 64  & k0: 10 i1: 50 i2: 2 j2: 64 k2: 10  &  &  & 46,1,47,31,0\\
bert\_100\_768 & False & I 100 J 768 K 100 & 216.95 & 1.13 & 1.13 & j0: 48 i1: 2 i2: 50 j2: 16  & i0: 2 k0: 5 j1: 768 i2: 50 k2: 20  &  &  & 73,8,50,31,0\\
bert\_3072\_100 & False & I 3972 J 100 K 3972 & 44.67 & 536.42 & 626.60 & i0: 2 load: C j0: 50 i1: 3 i2: 512 j2: 2  & i0: 6 load: C load: A j0: 50 k1: 3072 i2: 512 j2: 2  &  &  & 12,41,42,10,53\\
bicg & False & M 390, N 410 & 1.86 & 1.92 & 1.93 & i1: 2 i2: 195  & i1: 5 i2: 82  & j: 390 i: 410  & j1: 195 i2: 410 j2: 2  & 59,19,28,27,0\\
cnn & False & I 256 J 256 H 224 W 224 P 5 Q 5 & 307.78 & 7.30 & 9.68 & i0: 16 load: weight load: output j0: 256 load: input w0: 14 q0: 5 h1: 224 i2: 16 w2: 16 p2: 5  &  &  &  & 93,13,38,31,26\\
doitgen & False & NQ 40, NR 50, NP 60 & 54.05 & 5.46 & 2.71 & r0: 2 q0: 4 r1: 25 q2: 10 p2: 60  & q0: 4 s0: 30 r1: 50 q2: 10 p2: 60 s2: 2  & r0: 50 q0: 2 q1: 2 q2: 10 p2: 60  &  & 87,28,48,33,0\\
gemm & False & NI 200, NJ 220, NK 240 & 210.63 & 9.25 & 9.57 & j1: 55 i2: 200 j2: 4  & k0: 60 j1: 220 i2: 200 k2: 4  &  &  & 93,1,54,36,1\\
gemver & False & N 400 & 12.45 & 30.91 & 7.24 & i0: 2 j0: 25 i1: 10 i2: 20 j2: 16 & i0: 2 j0: 20 i1: 25 i2: 8 j2: 20 & i0: 2 i1: 2 i2: 100 & j0: 25 i1: 10 i2: 40 j2: 16  & 50,21,72,31,0\\
mvt & False & N 400 & 10.00 & 1.45 & 1.45 & i1: 200 i2: 2 j2: 400  & j1: 200 i2: 400 j2: 2  &  &  & 58,21,27,26,0\\
symm & False & M 200, N 240 & 236.56 & 8.14 & 7.19 &  &  &  &  & 95,10,73,54,0\\
syr2k & False & M 200, N 240 & 428.39 & 17.57 & 3.13 &  &  &  &  & 96,1,80,58,0\\
syrk & False & M 200, N 240 & 308.71 & 12.55 & 4.43 &  &  &  &  & 95,1,56,49,0\\
heat-3d & - & TSTEPS 100, N 40 & 131.33 & 35.09 & 0.99 & t: 100 k0: 38 i1: 38 j2: 38 k0: 38 i1: 38 j2: 38  &  &  &  & 32,28,44,14,0\\
jacobi-2d & - & TSTEPS 100, N 250  & 128.83 & 13.06 & 6.60 & t: 100 i1: 248 j2: 248 i1: 248 j2: 248  &  &  &  & 58,11,47,27,0\\
\midrule
Average &  &  & 152.66 & 59.96 & 22.82 &  &  &  &  & 68,13,50,34,2\\
Geo Mean &  &  & 68.88 & 5.96 & 2.88 &  &  &  &  & 62,,46,31,\\



\bottomrule

\end{tabular}
% \end{tabularx}
\caption{Comparison of the Throughput (GF/s) achieved with \framework, AutoDSE and NLP-DSE }

\label{tab:eval}
\end{adjustwidth}
\end{table*}





==> sources/table_var.tex <==
% \begin{table}[!htb]
\begin{table}[H]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{0.18\linewidth}p{0.82\linewidth}@{}}
\toprule
Set & Description \\
\midrule
$\mathcal{L},\mathcal{A},\mathcal{S}$ & the set of loops, arrays and statements \\
$\mathcal{S}_{1}$ & the set of statements alone in a loop body \\
$\mathcal{O}_s$ & the list of operations of the statements $s$ \\
% $\mathcal{O}_{s_{par}}$ & the operation which can be done in parallel, i.e., does not have any loop-carried dependence \\ 
$\mathcal{L}_s$ &  the set of nested loops which iterate the statement $s$ \\
$\mathcal{L}_s^{red}$ &  the set of reduction loops which iterate the statement $s$ \\
$\mathcal{C}_{a_d}$ & the set of loops which iterates the array $a$ at the dimension $d$ \\ 
$\mathcal{V}$ & Level of the strip mining, 0 for coarse-grained/sequential, 1 for pipeline and 2 for fine-grained unrolled \\
$AP_{a,d}$ & Array Partition for the array $a$ in dimension $d$ \\
% $d_l$ & the maximum dependency distance of the loop $l$ \\
\midrule
Variable & Description \\
\midrule

$tc_{l, level}$ & TC of the loop $l$ for the level of strip-mining \\
$loop_l\_UF$ & Coarse-grained unroll factor of the loop $l$ at level 0 of the strip-mining\\
$loop_l\_pip$  & Boolean to know if the loop $l$ is pipelined at level 1 of the strip-mining\\
$cache_l\_arr_a$ & Boolean to know if the array $a$ is transferred on-chip after the loop $l$ at level 0 of the strip-mining \\
\midrule
Constant & Description \\
\midrule
$TC_l$ & Trip Count of the loop $l$ before strip-mining \\
$II_l$ & II of the loop $l$ \\
$IL_{par}, IL_{red}$ & Iteration Latency of the operations without ($par$) and with ($red$) dependencies of the statement $s$\\
% $IL_{red}$ & Iteration Latency of the operations with dependencies of the statement $s$\\
$DSP_{s_{op}}$ & Number of DSP used for the statement $s$ for the operation $op$\\
$DSP_{available}$ & Number of DSP available for the FPGA used \\
$max_{part}$ & Maximum array partitioning defined by the user \\
$ft\_arr_a\_loop_l$ & Footprint of the array $a$ if transferred to on-chip before the loop $l$ \\
$reuse_{opt}$ & Boolean for optimistic reuse \\
\bottomrule
\end{tabular}%
% }
\caption{Overview of the sets, variables, and constants employed in formulating the NLP}
\label{tab:var}
\end{table}

% \vspace{-0.4cm}

==> sources/tablebis.tex <==
% % \vspace{-0.3cm}
% \begin{table}[H]
\begin{table}[H]
% \begin{table}[!htb]
% \vspace{-0.3cm}
% \footnotesize % TODO idk if i have right
\begin{adjustwidth}{-1in}{-1in}
    
\centering
\begin{tabular}{@{}l @{\hspace{-0.6mm}}rc  r @{\hspace{-0.6mm}} rr r  r @{}}
\toprule \\[-3.4ex]
& & &  \multicolumn{1}{l}{GF/s} & & \multicolumn{3}{l}{Perf. Impr. of ours framework vs.}  \\[-0.4ex]
\cmidrule{4-4}
\cmidrule{6-8}  \\[-3.4ex]

\textbf{Kernel} &  \textbf{TR} & \textbf{T} & 
% \textbf{AutoDSE} & \textbf{NLP-DSE} & 
\textbf{Ours} & & \textbf{A-DSE} & \textbf{N-DSE} & \textbf{S-HLS}   \\[-0.4ex]






\midrule
atax & 1 & D & 1.96 &  & 0.99x & 1.00x & 1.23x \\
atax & 0 & D & 1.86 &  & 0.98x & 1.00x & -\\


\midrule \\[-3.6ex]

2mm & 1 & D,P & 175.49 &  & 431.17x & 1.42x & 5.50x\\
2mm & 0 & D,P & 171.07 &  & 817.42x & 1.44x & -\\
3mm & 1 & D,P & 140.83 &  & 80.75x & 1.02x & 3.86x \\
3mm & 0 & D,P & 140.11 &  & 511.64x & 1.04x & - \\
bert\_100\_64 & 1 & D,P & 81.22 &  & 0.99x & 0.95x & -\\
bert\_100\_64 & 0 & D,P & 76.76 &  & 1.09x & 1.09x & -\\
bert\_100\_768 & 1 & D,P & 218.08 &  & 1.12x & 1.19x & -\\
bert\_100\_768 & 0 & D,P & 216.95 &  & 1.13x & 1.13x & -\\
bert\_100\_3072 & 1 & D,P & 241.59 &  & 1.21x & 1.21x & -\\
bert\_100\_3072 & 0 & D,P & 241.06 &  & 1.22x & 1.22x & -\\
gemm & 1 & D,P & 203.39 &  & 1.84x & 1.55x & 5.81x\\
gemm & 0 & D,P & 210.61 &  & 9.25x & 9.57x & -\\
\midrule \\[-3.6ex]
bicg & 1 & D,P & 1.96 &  & 1.97x & 1.97x & 1.18x\\
bicg & 0 & D,P & 1.86 &  & 1.92x & 1.93x & -\\
gemver & 1 & P & 17.62 &  & 4.58x & 1.74x & 9.39x\\
gemver & 0 & P & 15.01 &  & 37.28x & 8.73x & -\\
gesummv & 1 & D & 1.96 &  & 0.99x & 1.00x & 0.71x \\
gesummv & 0 & D,P & 1.81 &  & 0.97x & 0.97x & - \\
mvt & 1 & P & 13.24 &   & 1.70x & 1.70x & 1.26x\\
mvt & 0 & P & 9.75 &   & 1.42x & 1.42x & -\\

\midrule \\[-3.6ex]

bert\_3072\_100 & 1 & D,P,T & 314.89 &  & 21.85x & 24.29x & -\\
bert\_3072\_100 & 0 & D,P,T & 82.41 &  & 989.65x & 1,156.02x & -\\
cnn & 1 & D,P,T & 314.15 &   & 7.38x & 8.23x & -\\
cnn & 0 & D,P,T & 341.20 &  & 8.09x & 10.73x & -\\

\midrule \\[-3.6ex]

doitgen & 1 & D,P & 54.05 &  & 1.35x & 2.71x & -\\
doitgen & 0 & D,P & 54.05 &  & 5.46x & 2.71x & -\\
symm & 1 & D,P & 240.50 &  & 8.28x & 8.28x & 2,704.51x\\
symm & 0 & D,P & 240.55 &  & 8.28x & 7.32x & -\\
syr2k & 1 & D,P & 254.69 &  & 5.52x & 1.86x & 174.47x\\
syr2k & 0 & D,P & 429.34 &  & 17.61x & 3.14x & -\\
syrk & 1 & D,P & 161.20 &  & 6.55x & 2.32x & 358.95x\\
syrk & 0 & D,P & 333.03 &   & 13.54x & 4.78x & -\\
trmm & 1 & D,P & 148.53 &  & 8,345.10x & 8,312.42x & 2,376.91x \\
trmm & 0 & D,P & 130.90 &  & 7,362.68x & 7,333.85x & - \\

\midrule \\[-3.6ex]
Average &  & & 147.26 &  & \avgautodse  & \avgnlp & \avgscale \\
Geo Mean & & & 62.33 &  & \geoautodse  & \geonlp & \geoscale \\




\bottomrule

\end{tabular}
\caption{Comparison of the Throughput (GF/s) achieved with \framework, AutoDSE, NLP-DSE and Scale-HLS}

\label{tab:eval}
\end{adjustwidth}
% \vspace{-0.9cm}
\end{table}

% 




